Catch the Butterfly: Peeking into the Terms and Conflicts among SPDX Licenses

The widespread adoption of third-party libraries (TPLs) in software development has accelerated the creation of modern software. However, this convenience comes with potential legal risks. Developers may inadvertently violate the licenses of TPLs, leading to legal issues. While existing studies have explored software licenses and potential incompatibilities, these studies often focus on a limited set of licenses or rely on low-quality license data, which may affect their conclusions. To address this gap, there is a need for a high-quality license dataset that encompasses a broad range of mainstream licenses to help developers navigate the complex landscape of software licenses, avoid potential legal pitfalls, and guide solutions for managing license compliance and compatibility in software development. To this end, we conduct the first work to understand the mainstream software licenses based on term granularity and obtain a high-quality dataset of 453 SPDX licenses with well-labeled terms and conflicts. Specifically, we first conduct a differential analysis of the mainstream platforms to understand the terms and attitudes of each license. Next, we propose a standardized set of license terms to capture and label existing mainstream licenses with high quality. Moreover, we include copyleft conflicts and conclude the three major types of license conflicts among the 453 SPDX licenses. Based on these, we carry out two empirical studies to reveal the concerns and threats from the perspectives of both licensors and licensees. One study provides an in-depth analysis of the similarities, differences, and conflicts among SPDX licenses, revisits the usage and conflicts of licenses in the NPM ecosystem, and draws conclusions that differ from previous work. Our studies reveal some insightful findings and disclose relevant analytical data, which set the stage for further research.

==> Tables/NPM_test.tex <==
\begin{table}[]
\centering
\caption{Statistics on dependency conflicts and their impact}
% \footnotesize
\begin{tabular}{cccc}
\toprule
\begin{tabular}[c]{@{}c@{}}\textbf{Library} \\ \textbf{version}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Direct} \\ \textbf{dependencies}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Conflict} \\ \textbf{num/pro}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Affected indirect} \\ \textbf{dependencies}\end{tabular} \\ \hline
Lv1                                                        & 117,772                                                        & 27,462(23.32\%)                                             & 84,717(28.16\%)                                                           \\ 
Lv2                                                        & 117,772                                                        & 27,462(23.32\%)                                             & 84,717(28.16\%)                                                           \\ 
Lv3                                                        & 6,464                                                          & 290(4.5\%)                                                  & 2,371,899(96.57\%)                                                        \\ 
All                                                        & 3,391,572                                                      & 616,517(18.18\%)                                            & 5,549,335(33.41\%)                                                        \\ \toprule
\vspace{-3.0em}
\end{tabular}
\label{tab:NPM_test}
\end{table}

==> Tables/SCA.tex <==
% \begin{table*}[]
% \centering
% \caption{comparison among state-of-the-art SCA tools}
% \begin{tabular}{cccccccc}
% \toprule
% Tool      & Dependency & Vulnerability & License & Term & Attitude & Compliance & Free \\ \midrule
% Fossology & No         & No            & Yes     & No   & No       & No         & Yes  \\
% FOSSA     & Yes        & Yes           & Yes     & Yes  & No       & Suggestion & Yes  \\
% FOSSid    & Yes        & Yes           & Yes     & No   & No       & No         & No   \\
% FOSSEye   & Yes        & Yes           & Yes     & Yes  & Yes      & Yes        & No   \\
% Blackduck & Yes        & Yes           & Yes     & Yes  & Yes      & Unclear    & No   \\
% Snyk      & Yes        & Yes           & No      & No   & No       & No         & Yes  \\
% OWASP DC  & Yes        & Yes           & No      & No   & No       & No         & Yes  \\ \bottomrule
% \end{tabular}
% \label{SCA}
% \end{table*}



\begin{table*}
% \setlength{\abovecaptionskip}{0.cm}
% \setlength{\belowcaptionskip}{-0.cm}
\caption{Comparison among state-of-the-art SCA tools}
% \footnotesize
\begin{tabular}{cll}
SCA Tools & \multicolumn{1}{c}{Dependency}                                                                                                            & \multicolumn{1}{c}{License}                                                                     \\
FOSS      & \begin{tabular}[c]{@{}l@{}}Number: 862\\ Name: caniuse-lite and others\\ License: CC-BY-4.0 and others\\ Issues: 8 reminders\end{tabular} & \begin{tabular}[c]{@{}l@{}}Number: 19\\ Name: MIT and others\\ Term: 8 obligations\end{tabular} \\
Fossology & No results                                                                                                                                & \begin{tabular}[c]{@{}l@{}}Number: 7\\ Name: MIT and others\end{tabular}                        \\
Askalono  & No results                                                                                                                                & \begin{tabular}[c]{@{}l@{}}Number: 2\\ Name: MIT\end{tabular}                                   \\
ScanCode  & \begin{tabular}[c]{@{}l@{}}Number: 1355\\ Name: caniuse-lite and others\end{tabular}                                                      & \begin{tabular}[c]{@{}l@{}}Number: 16\\ Name: MIT\\ Copyright Info: 6\end{tabular}             
\end{tabular}
\label{tab:SCA}
\vspace{-1.0em}
\end{table*}





==> Tables/change_between_diffversion.tex <==
\begin{table}
\centering
\caption{Changes between versions of the same license}
% \footnotesize
\begin{tabular}{cccc}
\toprule
\begin{tabular}[c]{@{}c@{}}\textbf{Original}  \\ \textbf{license}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Changed} \\ \textbf{license}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Number of} \\ \textbf{changes}\end{tabular} & \textbf{Type}       \\ \toprule
BSD                                                          & BSD-3-Clause                                               & 367                                                          & Permissive \\
Apache                                                       & Apache   2.0                                               & 234                                                          & Permissive \\
BSD                                                          & BSD   2-Clause                                             & 200                                                          & Permissive \\
GPL-3.0                                                      & GPL-3.0+                                                   & 110                                                          & Copyleft   \\
GPL-3.0                                                      & AGPL-3.0                                                   & 89                                                           & Copyleft   \\
GPL                                                          & GPL-3.0                                                    & 78                                                           & Copyleft   \\
GPL-3.0                                                      & LGPL-3.0                                                   & 57                                                           & Copyleft   \\
MPL                                                          & MPL-2.0                                                    & 29                                                           & Copyleft   \\ \bottomrule
\vspace{-2.5em}
\end{tabular}
\label{tab:changes_diff}
\end{table}

==> Tables/comp_of_three_platform.tex <==


\begin{table}
\centering
% \vspace{-1.0em}
\setlength\tabcolsep{10pt} 
\caption{Comparison of the three license platforms}
% \footnotesize
\scalebox{0.68}{
\begin{tabular}{@{}ccccc@{}}
\toprule
\begin{tabular}[c]{@{}c@{}}Number of differences \\ in terms extraction\end{tabular} &
\begin{tabular}[c]{@{}c@{}}Choosealicense \\ (41 licenses )\end{tabular} & 
\begin{tabular}[c]{@{}c@{}}TLDRLegal   \\ (149 licenses)\end{tabular} & 
\begin{tabular}[c]{@{}c@{}}openEuler  \\ (254 licenses)\end{tabular} & 
\begin{tabular}[c]{@{}c@{}}Total \\  num \end{tabular} & 
\hline 
Sublicense                                                                           & 23                                                                       & 35                                                                    & 122                                                                  & 180   \\ \hline
Place Warranty                                                                       & 1                                                                        & 135                                                                   & 20                                                                   & 156   \\ \hline
Relicense                                                                            & 8                                                                        & 33                                                                    & 75                                                                   & 116   \\ \hline
Include Notice                                                                       & 15                                                                       & 27                                                                    & 74                                                                   & 116   \\ \hline
Private Use                                                                          & 0                                                                        & 63                                                                    & 40                                                                   & 103   \\ \hline
Give Credit                                                                          & 4                                                                        & 20                                                                    & 53                                                                   & 77    \\ \hline
Compensate for Damages                                                               & 7                                                                        & 28                                                                    & 40                                                                   & 75    \\ \hline
Use Patent Claims                                                                    & 1                                                                        & 38                                                                    & 33                                                                   & 72    \\ \hline
Use Trademark                                                                        & 7                                                                        & 21                                                                    & 38                                                                   & 66    \\ \hline
Include Copyright                                                                    & 1                                                                        & 31                                                                    & 15                                                                   & 47    \\ \hline
Include License                                                                      & 1                                                                        & 23                                                                    & 22                                                                   & 46    \\ \hline
State Changes                                                                        & 2                                                                        & 13                                                                    & 28                                                                   & 43    \\ \hline
Hold Liable                                                                          & 4                                                                        & 14                                                                    & 24                                                                   & 42    \\ \hline
Rename                                                                               & 3                                                                        & 7                                                                     & 21                                                                   & 31    \\ \hline
Include Original                                                                     & 4                                                                        & 8                                                                     & 18                                                                   & 30    \\ \hline
Disclose Source                                                                      & 2                                                                        & 6                                                                     & 14                                                                   & 22    \\ \hline
Commercial Use                                                                       & 0                                                                        & 7                                                                     & 10                                                                   & 17    \\ \hline
Contact Author                                                                       & 2                                                                        & 2                                                                     & 12                                                                   & 16    \\ \hline
Modify                                                                               & 0                                                                        & 1                                                                     & 13                                                                   & 14    \\ \hline
Include Install Instructions                                                         & 3                                                                        & 2                                                                     & 5                                                                    & 10    \\ \hline
Statically Link                                                                      & 0                                                                        & 2                                                                     & 4                                                                    & 6     \\ \hline
Distribute                                                                           & 0                                                                        & 1                                                                     & 3                                                                    & 4     \\ \hline
Total                                                                                & 88                                                                       & 517                                                                   & 684                                                                  & 1289  \\ \hline
\end{tabular}
}
\vspace{-2.0em}
\label{tab:comp_of_three_platform}
\end{table}


==> Tables/data_topten.tex <==
\begin{table}
\centering
\caption{The top 10 license pairs by number of changes}
% \footnotesize
\begin{tabular}{ccccc}
\toprule
\begin{tabular}[c]{@{}c@{}}\textbf{Original}  \\  \textbf{license}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Changed}  \\  \textbf{license}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Number   of} \\ \textbf{changes}\end{tabular} & \textbf{Proportion} & \\ \toprule
Unlicense                                                     & MIT                                                          & 17,390                                                          & 23.77\%                                                                          \\
ISC                                                           & MIT                                                          & 13,254                                                          & 18.11\%                                                                         \\
MIT                                                           & Unlicense                                                    & 4,925                                                           & 6.73\%                                                                            \\
MIT                                                           & ISC                                                          & 4,148                                                           & 5.67\%                                                                           \\
ISC                                                           & Unlicense                                                    & 2,518                                                           & 3.44\%                                                                                 \\
Unlicense                                                     & ISC                                                          & 2,428                                                           & 3.32\%                                                                                  \\
Unlicense                                                     & Apache   2.0                                                 & 1,934                                                           & 2.64\%                                                                             \\
MIT                                                           & Apache   2.0                                                 & 1,648                                                           & 2.25\%                                                                              \\
Apache   2.0                                                  & MIT                                                          & 1,021                                                           & 1.40\%                                                                              \\
ISC                                                           & Apache   2.0                                                 & 988                                                            & 1.35\%                                                                              \\ \midrule
\multicolumn{2}{c}{Total}                                                                                                    & 50,254                                                          & 68.68\%                                                                         \\ \toprule
\end{tabular}
\vspace{-2.0em}
\label{tab:data_topten}
\end{table}

==> Tables/distri_of_22_test.tex <==
\begin{table}[]
\centering
% \vspace{-1.0em}
\vspace{1pt}
\setlength{\tabcolsep}{1pt}

\caption{Distribution statistics of 22 terms in 453 licenses}

\footnotesize
% \resizebox{\textwidth}{!}{
\begin{tabular}{cccc}
\toprule
\textbf{Type}                          & \textbf{Term}                               & \textbf{Number of licenses}   & \textbf{Attitudes}   \\ \toprule
\multirow{19}{*}{Right}      & Distribute                         & 450                  & CAN         \\
                              & \multirow{2}{*}{Modify}            & \multirow{2}{*}{450} & CAN(437)    \\
                              &                                    &                      & CANNOT(13)  \\
                              & \multirow{2}{*}{Commercial Use}    & \multirow{2}{*}{432} & CAN(405)    \\
                              &                                    &                      & CANNOT(27)  \\
                              & \multirow{2}{*}{Place Warranty}    & \multirow{2}{*}{406} & CAN(10)     \\
                              &                                    &                      & CANNOT(396) \\
                              & \multirow{2}{*}{Hold Liable}       & \multirow{2}{*}{403} & CAN(17)     \\
                              &                                    &                      & CANNOT(386) \\
                              & \multirow{2}{*}{Use Trademark}     & \multirow{2}{*}{289} & CAN(13)     \\
                              &                                    &                      & CANNOT(276) \\
                              & Private Use                        & 262                  & CAN         \\
                              & \multirow{2}{*}{Sublicense}        & \multirow{2}{*}{210} & CAN(120)    \\
                              &                                    &                      & CANNOT(90)  \\
                              & \multirow{2}{*}{Relicense}         & \multirow{2}{*}{133} & CAN(18)     \\
                              &                                    &                      & CANNOT(115) \\
                              & \multirow{2}{*}{Use Patent Claims} & \multirow{2}{*}{106} & CAN(86)     \\
                              &                                    &                      & CANNOT(20)  \\
                              & Statically Link                    & 10                   & CAN         \\ \midrule
\multirow{11}{*}{Obligation} & Include License                    & 378                  & MUST        \\
                              & Include Copyright                  & 375                  & MUST        \\
                              & State Changes                      & 203                  & MUST        \\
                              & Give Credit                        & 154                  & MUST        \\
                              & Include Notice                     & 129                  & MUST        \\
                              & Disclose Source                    & 123                  & MUST        \\
                              & Compensate for Damages             & 54                   & MUST        \\
                              & Rename                             & 50                   & MUST        \\
                              & Include Original                   & 23                   & MUST        \\
                              & Contact Author                     & 13                   & MUST        \\
                              & Include Install Instructions       & 7                    & MUST        \\ \toprule
Total                         & 22                                 & 4,660                & 3  \\ \toprule      
\vspace{-2.8em}
\end{tabular}
\label{tab:distri_of_22_test}
\end{table}

==> Tables/distribute_topfive_license.tex <==
\begin{table*}
\centering
% \vspace{-1.0em}
\caption{Distribution comparison of the top five licenses for different library versions}
% \footnotesize
\begin{tabular}{ccc|ccc|ccc}
\toprule
\multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{All library version}\\  \textbf{(16,611,609)}\end{tabular}} & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{The earliest library version}\\ \textbf{(1,121,869)}\end{tabular}} & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{The latest library version}\\    \textbf{(1,121,869)}\end{tabular}} \\ \toprule
license                            & num                            & pro                          & license                               & num                              & pro                             & license                              & num                             & pro                             \\ \midrule
MIT                                & 9,091,827                        & 54.7\%                       & MIT                                   & 609,528                           & 54.3\%                          & MIT                                  & 631,626                          & 56.3\%                          \\
ISC                                & 2,379,369                        & 14.3\%                       & ISC                                   & 270,052                           & 24.0\%                          & ISC                                  & 259,076                          & 23.0\%                          \\
Apache 2.0                         & 1,833,461                        & 11.0\%                       & Unlicense                             & 125,719                           & 11.2\%                          & Unlicense                            & 110,183                          & 9.82\%                          \\
Unlicense                          & 1,633,749                        & 9.84\%                       & Apache 2.0                            & 43,914                            & 3.91\%                          & Apache 2.0                           & 46,984                           & 4.19\%                          \\
BSD-3-Clause                       & 254,040                         & 1.53\%                       & BSD-3-Clause                          & 9,917                             & 0.88\%                          & BSD-3-Clause                         & 10,664                           & 0.95\%                          \\ \toprule
Total                              & 15,192,446                       & 91.46\%                      & Total                                 & 1,059,130                          & 94.41\%                         & Total                                & 1,058,533                         & 94.35\%                         \\ \toprule
\end{tabular}
\vspace{-1.0em}
\label{tab:distribute_topfive_license}
\end{table*}

==> Tables/pairs_of_licenses_in_dependencies.tex <==
% \begin{table}[]
% \caption{Top-10 conflicted license pairs in direct dependencies for NPM}
% \scalebox{0.78}{
% \begin{tabular}{llc|llc|llc}
% \toprule
% \multicolumn{3}{c|}{\textbf{C1}}             & \multicolumn{3}{c|}{\textbf{C2}}              & \multicolumn{3}{c}{\textbf{C3}}                \\
% \midrule
% Parent & Dependency & \# & Parent & Dependency & \# & Parent & Dependency & \# \\
% \midrule
% MIT & CC0-1.0             & 109659 & MIT & Apache-2.0          & 3014374 & MIT & MPL-2.0                & 82200  \\
% MIT&GPL-3.0-or-later    & 24979  & ISC & Apache-2.0          & 1166969 & MIT & GPL-3.0-or-later       & 24979  \\
% MIT&GPL-2.0-or-later    & 22268  & Unlicense&MIT           & 97568   & ISC & MPL-2.0                & 22262  \\
% Apache-2.0 & CC0-1.0      & 20283  & MPL-2.0 & Apache-2.0      & 95712   & ISC & GPL-3.0-or-later       & 9477   \\
% Apache-2.0 & CC-BY-ND-4.0 & 14876  & MIT & MPL-2.0             & 82200   & LGPL-3.0-only & GPL-3.0-only & 1982   \\
% MIT & CC-BY-4.0           & 14847  & BSD-3-Clause & Apache-2.0 & 80831   & AAL & MPL-2.0                & 1606   \\
% CECILL-B & MIT            & 6347   & WTFPL & MIT               & 59052   & LGPL-3.0-only & MPL-2.0      & 1360   \\
% MPL-2.0 & CC0-1.0         & 6233   & MIT & WTFPL               & 53477   & BSD-3-Clause & MPL-2.0       & 1278   \\
% Apache-2.0 & GPL-3.0-only & 5178   & CC0-1.0&MIT             & 49628   & MIT & EPL-1.0                & 1223   \\
% MIT & CC-BY-3.0           & 5018   & MIT & Artistic-2.0        & 32539   & ISC & GPL-3.0-only           & 1193   \\
% \midrule
% Total         &            & 229688 & Total         &            & 4732350 & Total              &          & 147560 \\
% \bottomrule
% \end{tabular}}
% \label{tbl:topconflict}
% \end{table}

==> Tables/pl-cl_cl-cl.tex <==
% Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% % \usepackage{multirow}
% \begin{table}[]
% \centering
% \caption{The conflict combinations of attitudes under PL-CL and CL-CL}
% \begin{tabular}{@{}ccc@{}}
% \toprule[0.4mm]
% \multirow{2}{*}{PL-CL} & CAN-CANNOT  & CAN-MUST    \\ 
%                        & CANNOT-MUST & MUST-CANNOT \\ \cmidrule(r){1-1}
% CL-CL                  & CANNOT-MUST & MUST-CANNOT \\ \bottomrule[0.4mm]
% \end{tabular}
% \label{pl-cl&cl-cl}
% \end{table}

\begin{table}
\centering
\caption{Conflicting combinations under PL-CL and CL-CL}
% \footnotesize
\begin{tabular}{@{}ccc@{}}
\toprule

\textbf{Mode}                  & \multicolumn{2}{c}{\textbf{Conflicting Combination}} \\ \toprule
\multirow{2}*{PL-CL}                   & CAN-CANNOT  & CAN-MUST    \\ 
                          & CANNOT-MUST & MUST-CANNOT \\ \toprule
CL-CL & CANNOT-MUST & MUST-CANNOT \\ \toprule
\end{tabular}


\label{tab:pl-cl&cl-cl}
\vspace{-2.0em}
\end{table}

==> Tables/reason_of_difflabels.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}
%\vspace{-1.0em}
\caption{Statistics of the reasons for different extraction results}
\resizebox{\textwidth}{!}{
% \footnotesize
\begin{tabular}{cccccccc}
\toprule
\textbf{Reasons}                                                & \textbf{Classification}                                & \textbf{Platform a} & \textbf{Platform b} & \textbf{Platform c} & \multicolumn{3}{c}{\textbf{Number/Proportion}}                                   \\ \toprule
\multirow{3}{*}{Inconsistent with license description} & Explicitly described but not extracted          & 7              & 245         & 180       & \multicolumn{2}{c}{432 / 33.51\%}      & \multirow{3}{*}{641 / 49.73\%}     \\
                                                       & Not mentioned but extracted                     & 6              & 81          & 112       & \multicolumn{2}{c}{199 / 15.44\%}      &                                  \\
                                                       & Extraction is the exact opposite of description    & 0              & 8           & 2        & \multicolumn{2}{c}{10 / 0.78\%}        &                                  \\
                                                    \midrule[0.1mm]

\multirow{3}{*}{Inconsistent description of terms}     & Different coverage of the same term description    & 6              & 129         & 40        & 175 / 13.58\%          & \multicolumn{2}{c}{\multirow{3}{*}{197 / 15.28\%}} \\
                                                       & Multiple descriptions for the same term       & 0              & 17          & 0         & 17 / 1.32\%            & \multicolumn{2}{c}{}                             \\
                                                       & Same description extracted with different terms & 0              & 5           & 0         & 5 / 0.38\%             & \multicolumn{2}{c}{}                             \\
                                                       \midrule[0.1mm]
Unclear division of right and obligation               & NONE                                          & 0              & 4           & 3         & \multicolumn{3}{c}{7 / 0.54\%}                                            \\
Ignore of license name information                     & NONE                                          & 0              & 1           & 11        & \multicolumn{3}{c}{12 / 0.93\%}                                           \\
Inversion of License Subject                           & NONE                                          & 0              & 27          & 0         & \multicolumn{3}{c}{27 / 2.10\%}                                           \\ 
Inconsistent number of defined terms                       & NONE                                          & 69             & 0           & 336       & \multicolumn{3}{c}{405 / 31.42\%}                                         \\ \toprule
\multicolumn{2}{c}{Total/Proportion}                                                                   & 88 / 6.83\%      & 517 / 40.11\% & 684 / 53.06\%  & \multicolumn{3}{c}{1,289 / 100\%}                                          \\ \toprule
\end{tabular}}
\vspace{-1.0em}

\label{tab:reason_of_difflabels}
\end{table*}

